Path Planning with Uncertainty for Aircraft Under Threat of Detection from Ground-Based Radar

Mission planners for aircraft operating under threat of detection by ground-based radar systems are concerned with the probability of detection. Current path planning methods for such scenarios consider the aircraft pose, radar position, and radar parameters to be deterministic and known. This paper presents a framework for incorporating uncertainty in these quantities into a radar detection model that is used by a path planner. The developed path planner evaluates the radar detection risk in the presence of uncertainties and uses linear covariance analysis to efficiently generate error budgets. The error budgets identify the contribution of each source of uncertainty (e.g., sensor measurement noise, radar position uncertainty) to the overall variability in the probability of detection. The framework is applied to a modified visibility graph path planner that uses the detection risk and its variability to calculate path adjustments, which maintain the detection risk below a specified threshold. The results show that the framework is effective at providing actionable information to the mission planner that improves the final planned path and reduces the detection risk.

==> sections/AP_RadarJacobians.tex <==
%
% Section: Radar Model Jacobian
%
This appendix provides the Jacobians of $P_D$ as defined in \eqref{eq:pd_approx} with respect to the aircraft and radar states.
Further commentary on these partial derivatives is provided in \cite{rds,rds_ext}.

The perturbation of $P_D$ as defined in \eqref{eq:pd_partial_short} are expanded as
\begin{align}
    \delta P_{D} & \approx \partiald{P_D}{\mathcal{S}}\left(\partiald{\mathcal{S}}{R}\partiald{R}{\boldsymbol{x_{a}}}+\partiald{\mathcal{S}}{\sigma_{r}}\partiald{\sigma_{r}}{\boldsymbol{x_{a}}}\right) \Bigg\rvert_{\boldsymbol{\bar{x}_a}} \delta\boldsymbol{x_{a}} + \nonumber \\
                 & \qquad \partiald{P_D}{\mathcal{S}}\begin{bmatrix}\partiald{\mathcal{S}}{R}\partiald{R}{\boldsymbol{p_r^n}}+\partiald{\mathcal{S}} {\sigma_{r}}\partiald{\sigma_{r}}{\boldsymbol{p_r^n}} & \partiald{\mathcal{S}}{c_r} \end{bmatrix}\Bigg\rvert_{\boldsymbol{\bar{x}_r}}\delta\boldsymbol{x_{r}} \label{eq:pd_partial_long}\\
\end{align}

The partial derivative of $P_D$ \eqref{eq:pd_approx} with respect to $\mathcal{S}$ is given by
\begin{align}
\frac{\partial P_{D}}{\partial\mathcal{S}} & = \frac{\exp\left(-\left(\sqrt{-\ln P_{fa}}-\sqrt{\mathcal{S}+0.5}\right)^2\right)}{2\sqrt{\pi}\sqrt{\mathcal{S}+0.5}}.\label{eq:dp_dsnr}
\end{align}
The partial derivative of $\mathcal{S}$ \eqref{eq:SNR} with respect to $R$ is given by
\begin{align}
\frac{\partial\mathcal{S}}{\partial R} & =-c_r\frac{4 \sigma_r}{kR^{5}}
\end{align}
The partial derivative of $R$ \eqref{eq:range} with respect to $\boldsymbol{x_a}$ is given by
\begin{align}
\frac{\partial R}{\partial\boldsymbol{x_{a}}} & = \begin{bmatrix}\frac{\left(\boldsymbol{p_{a}-p_{r}}\right)^\intercal}{||\boldsymbol{p_{a}-p_{r}}||_{2}} & \boldsymbol{0_{1x3}}\end{bmatrix}.
\end{align}
The partial derivative of $\mathcal{S}$ \eqref{eq:SNR} with respect to $\sigma_r$ is given by
\begin{align}
\frac{\partial\mathcal{S}}{\partial\sigma_{r}} & = c_r\frac{1}{kR^{4}}.
\end{align}
The partial derivative of $R$ \eqref{eq:range} with respect to $\boldsymbol{p_r^n}$ is given by
\begin{equation}
    \partiald{R}{\boldsymbol{p_r^n}} = \frac{-\left(\boldsymbol{p_a} - \boldsymbol{p_r}\right)^\intercal}{||\boldsymbol{p_a} - \boldsymbol{p_r}||_2}.
\end{equation}
The partial derivative of $\mathcal{S}$ with respect to $c_r$ is given by
\begin{eqnarray}
    \partiald{\mathcal{S}}{c_r}&=&\frac{\sigma_r}{kR^4}.
\end{eqnarray}
The remaining partial derivatives in \eqref{eq:pd_partial_long} are $\partiald{\sigma_{r}}{\boldsymbol{x_a}}$ and $\partiald{\sigma_r}{\boldsymbol{p_r^n}}$ which are derived in the following subsection.

\subsection{Partial Derivatives of the Ellipsoid RCS Model}
The partial derivative of the ellipsoid RCS model \eqref{eq:rcs_ellipsoid} with respect to the $\boldsymbol{x_a}$ and $\boldsymbol{p_r^n}$ are given by
\begin{align}
    \partiald{\sigma_{r}}{\boldsymbol{x_a}} &= \partiald{\sigma_{r}}{\alpha} \partiald{\alpha}{\boldsymbol{x_a}} + \partiald{\sigma_{r}}{\phi} \partiald{\phi}{\boldsymbol{x_a}} \\
    \partiald{\sigma_r}{\boldsymbol{p_r^n}} &= \partiald{\sigma_r}{\alpha} \partiald{\alpha}{\boldsymbol{p_r^n}} + \partiald{\sigma_r}{\phi} \partiald{\phi}{\boldsymbol{p_r^n}}.
\end{align}
where the partial derivatives of the ellipsoid RCS model \eqref{eq:rcs_ellipsoid} with respect to the RCS azimuth $\alpha$ and elevation $\phi$ angles are given by 
\begin{eqnarray}
    \partiald{\sigma_{r}}{\alpha} &=& \frac{-2 \pi (abc)^2\sin(2\alpha)\kappa}{D^3} \\
    \partiald{\sigma_{r}}{\phi} &=& \frac{-2 \pi (abc)^2\left(b^2-a^2\right)\sin(\alpha)^2\sin(2\phi)}{D^3}
\end{eqnarray}
and
\begin{align}
    \kappa &= a^2\cos(\phi)^2+b^2\sin(\phi)^2-c^2 \\
    \textrm{D} &= \left(a \,\sin\alpha \, \cos \phi\right)^{2}+\left(b \,\sin\alpha\, \sin\phi\right)^{2}+\left(c\, \cos\phi\right)^{2}.
\end{align}

The partial derivatives of $\alpha$ and $\phi$ with respect to the radar position are given by
\begin{eqnarray}
    \partiald{\alpha}{\boldsymbol{p_r^n}} &=& \partiald{\alpha}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_r^n}} \\
    \partiald{\phi}{\boldsymbol{p_r^n}} &=& \partiald{\phi}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_r^n}}.
\end{eqnarray}

The partial derivative of the azimuth and elevation angle with respect to the radar position in the aircraft body frame $\boldsymbol{\rho_r^b}$ are given by
\begin{eqnarray}
    \partiald{\alpha}{\boldsymbol{\rho_r^b}} &=& \begin{bmatrix} \frac{-\rho_{ry}}{\rho_{rx}^2 + \rho_{ry}^2} & 
    \frac{\rho_{rx}}{\rho_{rx}^2 + \rho_{ry}^2} &
    0 \end{bmatrix} \\
    \partiald{\phi}{\boldsymbol{\rho_r^b}} &=& \begin{bmatrix} \frac{- \rho_{rx} \rho_{rz}}{\beta} & 
    \frac{- \rho_{ry} \rho_{rz}}{\beta}  &
    \frac{\sqrt{\rho_{rx}^2 + \rho_{ry}^2}}{\rho_{rx}^2 + \rho_{ry}^2 + \rho_{rz}^2} \end{bmatrix}
\end{eqnarray}
where
\begin{equation}
    \beta = \left(\rho_{rx}^2 + \rho_{ry}^2 + \rho_{rz}^2\right)\sqrt{\rho_{rx}^2 + \rho_{ry}^2}.
\end{equation}
The partial derivative of $\boldsymbol{\rho_r^b}$ with respect to $\boldsymbol{p_r^n}$ is given by  
\begin{eqnarray}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_r^n}} &=& T_n^b. 
\end{eqnarray}

Finally, the partial derivative of the $\alpha$ and $\phi$ with respect to $\boldsymbol{x_a}$ are given by 
\begin{eqnarray}
    \partiald{\alpha}{\boldsymbol{x_a}} &=& \partiald{\alpha}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}} \\
    \partiald{\phi}{\boldsymbol{x_a}} &=& \partiald{\phi}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}}
\end{eqnarray}
where 
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}} = \begin{bmatrix} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_a^n}} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}} \end{bmatrix}.
\end{equation}

The partial derivative of $\boldsymbol{\rho_r^b}$ with respect to the aircraft position in the NED frame is given by
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_a^n}} = -T_n^b
\end{equation}
where $T_n^b$ is defined in \eqref{eq:DCM_zyx}. The partial derivative of $\boldsymbol{\rho_r^b}$ with respect to the aircraft orientation is given by
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}} = \begin{bmatrix} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{11} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{12} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{13} \\
        \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{21} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{22} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{23} \\
        \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{31} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{33} \end{bmatrix}
\end{equation}
where
\begin{align}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{11} &= -(C{\phi_a} S{\psi_a} - C{\psi_a} S{\phi_a} S{\theta_a})p_{\Delta d} \nonumber \\
            & \quad -(S{\phi_a} S{\psi_a} + C{\phi_a} C{\psi_a} S{\theta_a})p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{12} &= C{\psi_a} S{\theta_a} p_{\Delta n} - C{\psi_a} C{\theta_a} S{\phi_a} p_{\Delta e} \nonumber  \\
            & \quad - C{\phi_a} C{\psi_a} C{\theta_a} p_{\Delta d} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{13} &= (C{\phi_a} C{\psi_a} + S{\phi_a}S{\psi_a}S{\theta_a})p_{\Delta e} \nonumber  \\
            & \quad - (C{\psi_a} S{\phi_a} - C{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta d} \nonumber  \\
            & \quad + C{\theta_a} S{\psi_a} p_{\Delta n} \\
%
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{21} &= (C{\phi_a} C{psi_a} + S{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta d} \nonumber \\
        & \quad + (C{\psi_a} S{\phi_a} - C{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{22} &= S{\psi_a} S{\theta_a} p_{\Delta n} - C{\phi_a} C{\theta_a} S{\psi_a} p_{\Delta d} \nonumber \\
        & \quad - C{\theta_a} S{\phi_a} S{\psi_a} p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{23} &= (C{\phi_a} S{\psi_a} - C{\psi_a}S{\phi_a}S{\theta_a})p_{\Delta e} \nonumber \\
        & \quad - (S{\phi_a} S{\psi_a} + C{\phi_a}C{\psi_a}S{\theta_a}) p_{\Delta d} \nonumber \\
        & \quad - C{\psi_a} C{\theta_a} p_{\Delta n} \\
%
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{31} &= C{\theta_a} S{\phi_a} p_{\Delta d} - C{\phi_a} C{\theta_a} p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} &= C{\theta_a} p_{\Delta n} + C{\phi_a} S{\theta_a} p_{\Delta d} + S{\phi_a} S{\theta_a} p_{\Delta e}   \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} &= 0
\end{align}
and
\begin{eqnarray}
    \boldsymbol{p_\Delta^n} &=& \boldsymbol{p_r^n}-\boldsymbol{p_a^n} \\
        &=& \begin{bmatrix} p_{\Delta n} & p_{\Delta e} & p_{\Delta d} \end{bmatrix}^\intercal.
\end{eqnarray}

\subsection{Combining Expressions for $A_{Pa}$ and $A_{Pr}$}
The partial derivatives calculated in the preceding subsections are combined to obtain an expression for $A_{Pa}$ and $A_{Pr}$ as
\begin{eqnarray}
    A_{Pa} &=& \begin{bmatrix} 
            -c_r\frac{2\text{exp}\left(-W^2\right)\left(\boldsymbol{p_{a}-p_{r}}\right)^\intercal}{kR^{6}\sqrt{\pi}\sqrt{\mathcal{S}+0.5}} & \boldsymbol{0_{1x3}}
            \end{bmatrix} \nonumber \\
           & & +
            c_r\frac{\exp\left(-W^2\right)}{2kR^{4}\sqrt{\pi}\sqrt{\mathcal{S}+0.5}} \frac{\partial \sigma_r}{\partial \boldsymbol{x_a}} \\
    A_{pr} &=& \frac{\exp\left(-W^2\right)}{2\sqrt{\pi}\sqrt{\mathcal{S}+0.5}} \nonumber \\
            & & \qquad \begin{bmatrix} \frac{4 c_r \sigma_r \left(\boldsymbol{p_a} - \boldsymbol{p_r}\right)^\intercal}{kR^{5}||\boldsymbol{p_a} - \boldsymbol{p_r}||_2} + \frac{c_r}{kR^{4}} \partiald{\sigma_{r}}{\boldsymbol{p_r^n}} & \frac{\sigma_r}{kR^4}\end{bmatrix}            
\end{eqnarray}
where
\begin{equation}
    W = \sqrt{-\ln P_{fa}}-\sqrt{\mathcal{S}+0.5}.
\end{equation}


==> sections/Appendices.tex <==
%
%  Section: RCS Azimuth and Elevation Angle
%
This appendix section provides the derivation for the RCS azimuth $\alpha$ and elevation $\phi$ angles used in the ellipsoid RCS model in \eqref{eq:rcs_ellipsoid}.
The RCS model used on this paper provides an expression for the RCS value as a function of the azimuth and elevation angles of the radar detection vector in the body frame of the aircraft.
The body frame $x$ and $y$ axes are shown as $b_x$ and $b_y$ in Fig. \ref{fig:radar_xy} and the body frame $z$ axis points out of the bottom of the aircraft.
Let the aircraft position in the NED frame and the aircraft attitude be defined as
\begin{eqnarray}
    \boldsymbol{p_a^n} &=& \begin{bmatrix} p_{an} & p_{ae} & p_{ad} \end{bmatrix}^\intercal \label{eq:pa} \\
    \boldsymbol{\Theta_a} &=& \begin{bmatrix} \phi_a & \theta_a & \psi_a \end{bmatrix}^\intercal \label{eq:theta_a}
\end{eqnarray}
and the radar position in the NED frame be defined as
\begin{equation}
    \boldsymbol{p_r^n} = \begin{bmatrix} p_{rn} & p_{re} & p_{rd}\end{bmatrix}^\intercal. 
\end{equation}
The position of the radar in the body frame of the aircraft is given by
\begin{equation}
\boldsymbol{\rho_r^b} = \begin{bmatrix} \rho_{rx} & \rho_{ry} & \rho_{rz} \end{bmatrix}^\intercal.
\end{equation}
The vector $\boldsymbol{\rho_r^b}$ is calculated using the aircraft pose and radar position by
\begin{equation}
    \boldsymbol{\rho_r^b} = T_n^b \left(\boldsymbol{p_r^n}-\boldsymbol{p_a^n}\right)
\end{equation}
where $T_n^b$ is the direction cosine matrix formed by the ZYX Euler angle sequence \cite{beard_randy_small_2012} given by
\begin{align}
    T_n^b = &\left[\begin{matrix}  C{\psi_a} C{\theta_a} & -C{\phi_a} S{\psi_a} + C{\psi_a} S{\phi_a} S{\theta_a}  \\
                C{\theta_a} S{\psi_a} & C{\phi_a} C{\psi_a} + S{\phi_a} S{\psi_a} S{\theta_a}  \\
                -S{\theta_a} & C{\theta_a} S{\phi_a} \end{matrix}\right.\nonumber \\
        & \qquad \qquad \qquad \qquad \left.\begin{matrix}
        S{\phi_a} S{\psi_a} + C{\phi_a}C{\psi_a}S{\theta_a} \\
        -C{\psi_a} S{\phi_a} + C{\phi_a} S{\psi_a} S{\theta_a} \\
        C{\phi_a} C{\theta_a} \end{matrix}\right] \label{eq:DCM_zyx}
\end{align}
and $\textrm{S}\cdot$ and $\textrm{C}\cdot$ are the $\sin(\cdot)$ and $\cos(\cdot)$ functions.

The RCS azimuth angle is the angle from the body frame $x$ axis to the projection of the radar detection vector into the $x$-$y$ plane of the body frame given by 
\begin{eqnarray}
    \alpha &=& \arctan\left(\frac{\rho_{ry}}{\rho_{rx}}\right).
\end{eqnarray}
The RCS elevation angle $\phi$ is the angle from the $x$-$y$ plane in the body frame of the aircraft to the radar detection vector with a positive angle towards the bottom of the aircraft given by
\begin{eqnarray}
    \phi &=& \arctan\left(\frac{\rho_{rz}}{\sqrt{(\rho_{rx})^2+(\rho_{ry})^2}}\right).
\end{eqnarray}





==> sections/Introduction.tex <==
\paperplan{Intro Paragrphs / Motivation}
{
    \begin{itemize}
        \item Mission planners plan paths for aircraft under threat of detection from ground-based radar systems
        \item Example missions include ....
        \item Current planning methods assume deterministic states
        \item Our previous papers provide a framework for incorporating uncertainty
        \item Contribution overview: Path planner with uncertainty for radar detection threat
    \end{itemize}
}

Aircraft mission planners are tasked with planning paths for aircraft operating under threat of detection by ground-based radar systems.
Example missions include reconnaissance \cite{Ceccarelli_micro_uav}, radar counter-measure deployment \cite{larson_path_nodate,xiao-wei_path_2010}, and combat operations \cite{kabamba_optimal_2012}.
Mission planners for such scenarios are primarily interested in the probability of being detected by a radar system.
The probability of detection is a function of the aircraft position and orientation (pose), radar position, radar system parameters, and the physical characteristics of the aircraft (e.g. radar cross section, material). 

Current radar detection path planning methods consider the quantities used to compute the probability of detection to be deterministic and known \cite{mcfarland_motion_1999,bortoff_path_2000,chandler_uav_2000,pachter_optimal_2001,moore_radar_2002,jun_path_2003,larson_path_nodate,kabamba_optimal_2012,xiao-wei_path_2010}.
In practice, each of these quantities has inherent uncertainty.
The aircraft pose, for example, is estimated by a navigation filter using measurements that are noisy and biased \cite{savage_strapdown_2000, farrell_aided_2008, grewal_global_2020}.
Whereas, the radar position and radar parameters are estimated using gathered intelligence.

Previous work has provided methods to incorporate uncertainty in aircraft and radar states into the probability of detection \cite{rds,rds_ext}.
This paper describes the incorporation of these methods into a path planning algorithm.
The path planner models an inertial navigation system (INS) to obtain the aircraft state uncertainty along a candidate trajectory.
The aircraft state and radar position are used to compute the nominal probability of detection and the aircraft and radar state uncertainty are used to compute the variability of the probability of detection.
% The aircraft state, aircraft state uncertainty, and radar uncertainty are used to compute the nominal probability of detection and the variability of the probability of detection.
The probability of detection and its variability are then used to inform a path planning algorithm.

\paperplan{Literature Reivew}
{
    \begin{itemize}
        \item Radar detection literature review (minor)
        \item \cite{rds, rds_ext} to incorporate uncertainty
        \item Radar detection path planning
        \item Visibility graph planning
        \item Need to incorporate uncertainty
        \item Path planning with uncertainty
        \item Inertial navigation
        \item LinCov
    \end{itemize}
}

The target detection literature for ground-based radar systems provides high-fidelity radar detection models.
Marcum \cite{marcum_statistical_1960} expresses the target detection probability for a single-pulse radar detection model as a nonlinear function of the radar position and parameters, target pose, and radar cross section (RCS).
Swerling \cite{swerling_probability_1954} extends the work by Marcum to include a multiple-pulse radar model and fluctuating targets.
Mahafza \cite{mahafza_matlab_2003} uses the expressions from Marcum and Swerling and includes considerations for modeling modern radar systems and provides expressions for common RCS models as a function of the aircraft pose relative to the radar.

Current path planning methods use a variety of approaches to estimate the detection risk along candidate paths.
% These approaches include proxies for the probability of detection from \cite{marcum_statistical_1960,swerling_probability_1954,mahafza_matlab_2003} to simplify the computation for the path planning algorithm.
These approaches include integrated inverse range models \cite{bortoff_path_2000,chandler_uav_2000,pachter_optimal_2001,larson_path_nodate,xiao-wei_path_2010}, peak/aggregate RCS \cite{moore_radar_2002}, radar range equation \cite{mcfarland_motion_1999}, and a logistic function approximation with consolidated radar parameters \cite{kabamba_optimal_2012}. 
With the exception of \cite{kabamba_optimal_2012}, these methods do not attempt to quantify the probability of detection which is necessary for the mission planning scenario introduced above.
Furthermore, none of these approaches, including those presented by Mahafza, account for uncertainty in the aircraft pose, radar position, and radar parameters.

Aircraft operating in radar detection regions are often equipped with an aided inertial navigation system (INS).
Such a system uses measurements from an inertial measurement unit (IMU) and aiding sources, such as GPS, to estimate the aircraft pose and pose covariance \cite{savage_strapdown_2000,grewal_global_2020,farrell_aided_2008}.
A common filtering technique for an aided INS is the Extended Kalman Filter (EKF) \cite{maybeck_stochastic_1994,brown_kalman}.  
This paper uses the covariance propagation equations for an  EKF to estimate the aircraft state covariance.
A challenge with modeling an EKF for an INS in a path planner is that the EKF covariance propagation equation requires the generation of IMU measurements along each candidate path at a high frequency. 
This challenge is mitigated in the current work through the use of an efficient IMU measurement generation method using the path geometry \cite{asg}.

The aircraft state covariance estimation and radar detection model presented in this paper can be applied to a wide variety of path planners.
One approach in the radar detection path planning literature is to use a two-stage algorithm that first generates a piece-wise linear path and then adjust the path to meet mission objectives \cite{bortoff_path_2000,jun_path_2003,chandler_uav_2000}.
This type of approach is useful for the present work because the IMU measurement generation method in \cite{asg} takes, as an input, a piece-wise linear path and produces a smooth flyable trajectory with associated IMU measurements.

The INS and radar detection model presented in this paper are used to obtain an estimate of the variability of the probability of detection along a candidate path.
However, they do not provide a way to compare the contribution of each source of uncertainty.
This is traditionally accomplished using Monte Carlo analysis and error budgets [citations].
In this approach, a Monte Carlo analysis is executed for each source of uncertainty where the source in question is the only error source activated.
The results from each Monte Carlo run are combined into an error budget that shows a graphical comparison of how each source of uncertainty contributes to the overall variability of the quantity of interest (i.e. probability of detection).
The Monte Carlo approach is computationally prohibitive because it requires a large number of simulations (500+) for each source of uncertainty.
An alternative method is to use Linear Covariance analysis \cite{maybeck_stochastic_1994,christensen_2014,christensen2021closedloop} which produces the same statistical information as Monte Carlo analysis in a single run. 


% The algorithms include optimal control policies \cite{kabamba_optimal_2012,xiao-wei_path_2010,pachter_optimal_2001}, trajectory optimization \cite{moore_radar_2002,larson_path_nodate}, potential field \cite{mcfarland_motion_1999}, and two-stage algorithms that create a piece-wise linear path and then adjust the path to meet objectives  \cite{bortoff_path_2000,jun_path_2003,chandler_uav_2000}.
% The primary application presented in this work uses a modified Visibility
% Graph \cite{lozano-perez_algorithm_1979}. This method was chosen
% because the radars can be modeled as polygons which is ideal
% for Visibility Graph path planning. The resulting piece-wise linear
% path is then smoothed using \cite{asg}. The probability
% of detection and its variability can then be accurately estimated along the entire trajectory
% to determine if the path is valid. Using the validity information
% the path can be adjusted to meet the mission requirements.

\paperplan{Contributions}
{
   \\ Come back to this 
}

The primary contribution of this paper is a method to incorporate aircraft and radar state uncertainty into the radar detection model of a path planner.
The aircraft state covariance is estimated by an INS with nominal states and inertial measurements generated using the ASG method from \cite{asg}.
The aircraft and radar state covariances are incorporated in the radar detection model using the methods presented in \cite{rds, rds_ext}.
The resulting nominal probability of detection and variability of the probability of detection are used by the path planner to determine the validity of candidate paths.
This paper demonstrates the path planning application through the use of a two-stage algorithm that uses a modified Visibility Graph path planner \cite{lozano-perez_algorithm_1979} to generate a piece-wise linear path.
Then the path is adjusted according to the radar detection information to meet the mission requirements.

The resulting trajectory is evaluated using Linear Covariance analysis to generate error budgets for the sources of uncertainty.
It is shown that a mission planner can use information from an error budget to make actionable design decisions about the quality of sensors, or radar intelligence requirements.
The result is a reduction of the variability in the probability of detection and an improvement in the planned path (i.e. shorter length).

The remainder of this paper is organized as follows.
Section \ref{sec:radar_model} presents the radar detection model which provides an expression for the probability of detection, the linearization of the model, and the incorporation of aircraft and radar state uncertainty.
The aircraft state uncertainty is computed using an aided INS as described in Section \ref{sec:ins_model}.
Section \ref{sec:lincov} describes the linear covariance model and the method for generating error budgets.
Section \ref{sec:vgraph} describes the path planner that incorporates these components and the results of the path planner are provided in Section \ref{sec:Results}.



